Pulsar Observations with the Fermi Large Area Telescope

The Large Area Telescope (LAT) on Fermi, launched on 2008 June 11, is a space telescope to explore the high energy gamma-ray universe. The instrument covers the energy range from 20 MeV to 300 GeV with greatly improved sensitivity and ability to localize gamma-ray point sources. It detects gamma-rays through conversion to electron-positron pairs and measurement of their direction in a tracker and their energy in a calorimeter. This thesis presents the gamma-ray light curves and the phase-resolved spectral measurements of radio-loud gamma-ray pulsars detected by the LAT. The measurement of pulsar spectral parameters (i.e. integrated flux, spectral index, and energy cut-off) depends on the instrument response functions (IRFs). A method developed for the on-orbit validation of the effective area is presented using the Vela pulsar. The cut efficiencies between the real data and the simulated data are compared at each stage of the background rejection. The results are then propagated to the IRFs, allowing the systematic uncertainties of the spectral parameters to be estimated. The last part of this thesis presents the discoveries, using both the LAT observations and the radio and X ephemeredes, of new individual gamma-ray pulsars such as PSR J0205+6449, and the Vela-like pulsars J2229+6114 and J1048-5832. Timing and spectral analysis are investigated in order to constrain the gamma-ray emission model. In addition, we discuss the properties of a large population of gamma-ray pulsars detected by the LAT, including normal pulsars, and millisecond pulsars.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `babelbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\input{englbst}
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `babelbst.tex'.


==> biblio/babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `babelbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\input{englbst}
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `babelbst.tex'.


==> diagram/exemple_diag.tex <==

\begin{minipage}[b][1.3\totalheight][c]{15cm}
 \begin{center} \footnotesize
    \begin{minipage}[][][c]{4.5cm}
    \begin{center} 
      \setlength{\unitlength}{1mm}
      \begin{fmfgraph}(40,20)
	\fmfright{h2}
	\fmfleft{b1}
	\fmf{fermion}{b1,h2} 
      \end{fmfgraph}
    \end{center}
  \end{minipage}
  = 
  \begin{minipage}[][][c]{4.5cm}
    \begin{center} 
      \setlength{\unitlength}{1mm}
      \begin{fmfgraph}(40,20)
	\fmfright{h2}
	\fmfleft{b1}
	\fmf{dashes_arrow}{b1,h2} 
      \end{fmfgraph}
    \end{center}
  \end{minipage}
  +  
  \begin{minipage}[][][c]{4.5cm}
   \begin{center} 
      \setlength{\unitlength}{1mm}
      \begin{fmfgraph*}(40,10)
	\fmfstraight
	\fmfbottom{h,b,c}
	\fmftop{d}
	\fmf{dashes_arrow}{h,b}
	\fmf{fermion}{b,c}
	\fmf{wiggly,label=$\sigma \omega$}{b,d}
	\fmf{fermion}{d,d}
      \end{fmfgraph*}
      \vspace{1cm}
      \setlength{\unitlength}{1mm}
      \begin{fmfgraph}(40,10)
	\fmfstraight
	\fmfbottom{h,b,c}
	\fmf{dashes_arrow}{h,b}
	\fmf{fermion}{b,c}
	\fmf{fermion}{b,b}
      \end{fmfgraph}
    \end{center}
  \end{minipage}\end{center}
  \end{minipage}


==> englbst.tex <==
%%
%% This is file `englbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `englbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `englbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}
\def\bbletal{et~al} % Piste sijoitetaan tarvittaessa per^^e4^^e4n!
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{first}            \def\bblfirsto{1st}
\def\bblsecond{second}          \def\bblsecondo{2nd}
\def\bblthird{third}            \def\bblthirdo{3rd}
\def\bblfourth{fourth}          \def\bblfourtho{4th}
\def\bblfifth{fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}
\def\bblins{in} % Oma lis^^e4ys: "in" series.
\def\bblinj{in} % Oma lis^^e4ys: "in" journal.
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `englbst.tex'.


==> figures/fermi_lat_gbm.tex <==
\subfigure[LAT]{\includegraphics[scale=0.65]{figures/c3_LAT.jpg}}
\subfigure[GBM]{\includegraphics[scale=0.65]{figures/c3_GBM.jpg}}

==> figures/neutron_star.tex <==
\subfigure[Structure possible d'une étoile à neutrons.]{\includegraphics[scale=1.0]{figures/c1_neutron_star_structure.jpg}}
\subfigure[Masses d'étoiles à neutrons.]{\includegraphics[scale=0.5]{figures/c1_mass_ns.jpg}}

==> figures/pulsepar_figure.tex <==
\subfigure[Distribution $\delta - \Delta$]{\includegraphics[scale=0.4]{figures/c9_radiolag_psep.pdf}}
\subfigure[Distribution $E_{Cutoff} - B_{LC}$]{\includegraphics[scale=0.4]{figures/c9_CutOffvsBlc.pdf}}


==> part1/conclusion.tex <==
\chapter*{Conclusion} 

[Conclusion de la partie 1] 



==> part1/introduction.tex <==
\chapter*{Introduction} 

[Ceci est une introduction pour la partie I.] 


==> part1/table1.tex <==
\begin{landscape}
%%\begin{table*}
\begin{center}
%\begin{scriptsize}
\begin{tiny}
\tablefirsthead{\hline
\hline
PSR	&	PSRJ	& $\frac{\sqrt{\dot{E}}}{d^2}$ & $\dot{E}$ 	& $d$  & $S_{1400}$	& $S_{400}$ & Cluster, & Optical & EGRET & EgretDist ($^\circ$) &  TeV & Notes 		\\
&		& \% of Vela 	&(erg/s)	& (kpc)	& (mJy)	& (mJy) & Galaxy & X-ray & nearby & & assoc. &	\\
\hline}
\tablehead{\multicolumn{13}{l}{\small \sl continued from previous page}\\
\hline
\hline
PSR	&	PSRJ	& $\frac{\sqrt{\dot{E}}}{d^2}$ & $\dot{E}$ 	& $d$  & $S_{1400}$	& $S_{400}$ & Cluster, & Optical & EGRET & EgretDist ($^\circ$) &  TeV & Notes 		\\
&		& \% of Vela 	&(erg/s)	& (kpc)	& (mJy)	& (mJy) & Galaxy & X-ray & nearby & & assoc. &	\\
\hline}
\bottomcaption{Pulsars being timed for the Fermi Large Area Telescope (all known pulsars with $\dot E > 10^{34}$ ergs/s), 
ordered by $\sqrt{\dot E}/d^2$, where $\dot E$ is the spin-down energy loss rate and $d$ is the distance. $\sqrt{\dot E}/d^2$ 
as an indicator of expected gamma flux suffers many large uncertainties (see text). $S_{1400}$ and $S_{400}$ are the radio 
flux intensities at $1400$ MHz and $400$ MHz, respectively.``Cluster, Galaxy'' is the name of the globular cluster or the 
host galaxy, if the pulsar is in one. ``np'' means that the source is observed in X-rays, but not pulsed. If the pulsar 
is located less than $2$\degr \ away from a $3^{rd}$ EGRET catalog source \citep{3rdcatalog}, the EGRET name and the angular 
distance are listed. The asterisk (*) indicates that the 3EG source has more than one possible counterpart in the table. 
The TeV associations are taken from \citet{HESScatalog}, available at http://www.mpi-hd.mpg.de/hfm/HESS/public/HESS\_catalog.htm, 
and from MILAGRO: \citep{Milagro}. Nearby pulsar wind nebulae (PWN) are noted in the last column \citep{KRH04,MSER04}. 
The data in the first 8 columns were obtained from the ATNF database except for the radio flux densities with the 
superscripts \textit{a}: F. Camilo, private communication, \textit{b}: \citet{JBK03}, \textit{c}: \citet{KCM98}, \textit{d}: 
\citet{RTJ96}, \textit{e}: \citet{DALM01}, \textit{f}: \citet{CLF00}. This table is 
available in electronic form at the CDS via anonymous ftp to cdsarc.u-strasbg.fr (130.79.128.5) 
or via http://cdsweb.u-strasbg.fr/cgi-bin/qcat?J/A+A/}
\tabletail{\multicolumn{13}{r}{\small \sl continuing next page\ldots}\\}
\tablelasttail{\hline}
\par
\begin{supertabular}{ccccccccccccc}
\hline
\hline
B0833$-$45 & J0835$-$4510 & 100. & 6.9e+36 & 0.3 & 1100. & 5000. &    & OX & 3EG J0834$-$4511 & 0.34 & Vela & G263.9$-$3.3, Vela X \\ 
J0633+1746 & J0633+1746 & 22. & 3.3e+34 & 0.2 & --- & --- &    & OX & 3EG J0633+1751 & 0.24 &   & G195.1+4.3, Geminga \\ 
B0531+21 & J0534+2200 & 17. & 4.6e+38 & 2.0 & 14. & 646. &    & OX & 3EG J0534+2200 & 0.13 & Crab & G184.6$-$5.8, Crab, SN1054 \\ 
J0437$-$4715 & J0437$-$4715 & 14. & 1.2e+34 & 0.2 & 142. & 550. &    &  X &   &   &   & G253.4$-$42.0 \\ 
B0656+14 & J0659+1414 & 7.42 & 3.8e+34 & 0.3 & 3.70 & 6.50 &    & OX &   &   &   & Monogem Ring \\ 
B0743$-$53 & J0745$-$5353 & 5.37 & 1.1e+34 & 0.2 & --- & 23. &    &    &   &   &   &   \\ 
J0034$-$0534 & J0034$-$0534 & 1.90 & 3.0e+34 & 0.5 & 0.61 & 17. &    &    &   &   &   &   \\ 
J0205+6449 & J0205+6449 & 1.62 & 2.7e+37 & 3.2 & 0.04 & --- &    &  X &   &   &   & G130.7+3.1, 3C 58, SN1181 \\ 
J0613$-$0200 & J0613$-$0200 & 1.58 & 1.3e+34 & 0.5 & 1.40 & 21. &    &    &   &   &   &   \\ 
J1747$-$2958 & J1747$-$2958 & 1.25 & 2.5e+36 & 2.0 & { 0.07}$^{a}$ & --- &    &    & 3EG J1744$-$3011 (*) & 0.84 & HESS J1745$-$303 & G359.23$-$0.82, Mouse \\ 
B1706$-$44 & J1709$-$4429 & 1.11 & 3.4e+36 & 2.3 & 7.30 & 25. &    &  X & 3EG J1710$-$4439 & 0.18 &   & G343.1$-$2.3 \\ 
B1055$-$52 & J1057$-$5226 & 1.06 & 3.0e+34 & 0.7 & --- & 80. &    &  X & 3EG J1058$-$5234 & 0.12 &   &   \\ 
J1740+1000 & J1740+1000 & 0.99 & 2.3e+35 & 1.2 & 9.20 & 3.10 &    &    &   &   &   &   \\ 
B1951+32 & J1952+3252 & 0.98 & 3.7e+36 & 2.5 & 1.00 & 7.00 &    &    &   &   &   & G69.0+2.7, CTB 80 \\ 
J1357$-$6429 & J1357$-$6429 & 0.90 & 3.1e+36 & 2.5 & 0.44 & --- &    &  X &   &   &   &   \\ 
J1833$-$1034 & J1833$-$1034 & 0.84 & 3.4e+37 & 4.7 & 0.07 & --- &    &    &   &   & HESS J1833$-$105 & G21.5$-$0.9 \\ 
B1509$-$58 & J1513$-$5908 & 0.76 & 1.8e+37 & 4.2 & 0.94 & 1.50 &    &  X &   &   & HESS J1514$-$591 & G320.4$-$1.2, MSH 15-52 \\ 
B1257+12 & J1300+1240 & 0.74 & 1.9e+34 & 0.8 & 2.00 & 20. &    &  np &   &   &   &   \\ 
J1524$-$5625 & J1524$-$5625 & 0.73 & 3.2e+36 & 2.8 & 0.83 & --- &    &    &   &   &   &   \\ 
J1531$-$5610 & J1531$-$5610 & 0.69 & 9.1e+35 & 2.1 & 0.60 & --- &    &    &   &   &   &   \\ 
B1046$-$58 & J1048$-$5832 & 0.60 & 2.0e+36 & 2.7 & 6.50 & --- &    &    & 3EG J1048$-$5840 & 0.14 &   & G287.4+0.58 \\ 
B0355+54 & J0358+5413 & 0.56 & 4.5e+34 & 1.1 & 23. & 46. &    &    &   &   &   &   \\ 
J0940$-$5428 & J0940$-$5428 & 0.50 & 1.9e+36 & 3.0 & 0.66 & --- &    &    &   &   &   &   \\ 
J1930+1852 & J1930+1852 & 0.44 & 1.2e+37 & 5.0 & 0.06 & --- &    &  X & 3EG J1928+1733 & 1.46 &   & G54.1+0.3 \\ 
B1259$-$63 & J1302$-$6350 & 0.37 & 8.2e+35 & 2.8 & 1.70 & --- &    &  np &   &   & HESS J1302$-$638 &   \\ 
J0834$-$4159 & J0834$-$4159 & 0.36 & 9.9e+34 & 1.7 & 0.19 & --- &    &    &   &   &   &   \\ 
J1909$-$3744 & J1909$-$3744 & 0.36 & 2.2e+34 & 1.1 & --- & { 3.}$^{b}$ &    &    &   &   &   &   \\ 
B0906$-$49 & J0908$-$4913 & 0.35 & 4.9e+35 & 2.5 & 10. & 28. &    &    &   &   &   & G270.3$-$1.0 \\ 
J1509$-$5850 & J1509$-$5850 & 0.34 & 5.2e+35 & 2.6 & 0.15 & --- &    &    &   &   &   &   \\ 
B1823$-$13 & J1826$-$1334 & 0.34 & 2.8e+36 & 3.9 & 2.10 & --- &    &  np & 3EG J1826$-$1302 (*) & 0.55 & HESS J1825$-$137 & G18.0$-$0.7 \\ 
J1809$-$1917 & J1809$-$1917 & 0.34 & 1.8e+36 & 3.5 & 2.50 & --- &    &  np &   &   & HESS J1809$-$193 &   \\ 
J0538+2817 & J0538+2817 & 0.32 & 4.9e+34 & 1.5 & 1.90 & 8.20 &    &  X &   &   &   & S147 \\ 
J1811$-$1925 & J1811$-$1925 & 0.32 & 6.4e+36 & 5.0 & --- & --- &    &  X &   &   & HESS J1809$-$193 & G11.2$-$0.3, SN 386 \\ 
J1420$-$6048 & J1420$-$6048 & 0.31 & 1.0e+37 & 5.6 & 0.90 & --- &    &  X & 3EG J1420$-$6038 & 0.17 & HESS J1420$-$607 & G313.6+0.3, Kookaburra \\ 
B1800$-$21 & J1803$-$2137 & 0.31 & 2.2e+36 & 3.9 & 7.60 & 23. &    &  np &   &   & HESS J1804$-$216 &   \\ 
J1046+0304 & J1046+0304 & 0.30 & 1.4e+34 & 1.1 & 0.30 & --- &    &    &   &   &   &   \\ 
B0114+58 & J0117+5914 & 0.30 & 2.2e+35 & 2.2 & 0.30 & 7.60 &    &    &   &   &   &   \\ 
J2229+6114 & J2229+6114 & 0.28 & 2.2e+37 & 7.2 & 0.25 & --- &    &  X & 3EG J2227+6122 & 0.54 &   & G106.6+3.1 \\ 
J1718$-$3825 & J1718$-$3825 & 0.28 & 1.2e+36 & 3.6 & 1.30 & --- &    &    & 3EG J1714$-$3857 & 1.18 & HESS J1718$-$385 &   \\ 
B1727$-$33 & J1730$-$3350 & 0.27 & 1.2e+36 & 3.5 & 3.20 & 9.20 &    &    & 3EG J1734$-$3232 & 1.57 &   &   \\ 
B0740$-$28 & J0742$-$2822 & 0.27 & 1.4e+35 & 2.1 & 15. & 296. &    &    &   &   &   &   \\ 
J1617$-$5055 & J1617$-$5055 & 0.27 & 1.6e+37 & 6.8 & { 0.5}$^{c}$ & --- &    &  X &   &   & HESS J1616$-$508 &   \\ 
J1843$-$1113 & J1843$-$1113 & 0.27 & 6.0e+34 & 1.7 & 0.10 & --- &    &    &   &   &   &   \\ 
J2129$-$5721 & J2129$-$5721 & 0.26 & 2.3e+34 & 1.4 & 1.40 & 14. &    &    &   &   &   &   \\ 
J1124$-$5916 & J1124$-$5916 & 0.26 & 1.2e+37 & 6.5 & 0.08 & --- &    &  X &   &   &   & G292.0+1.8, MSH 11$-$54 \\ 
J1846$-$0258 & J1846$-$0258 & 0.25 & 8.1e+36 & 6.0 & --- & --- &    &  X &   &   & HESS J1846$-$029 & G29.7$-$0.3, Kes 75 \\ 
J1913+1011 & J1913+1011 & 0.24 & 2.9e+36 & 4.8 & 0.50 & --- &    &    &   &   & HESS J1912+101 &   \\ 
J1911$-$1114 & J1911$-$1114 & 0.23 & 1.2e+34 & 1.2 & 0.50 & 31. &    &    & 3EG J1904$-$1124 & 1.96 &   &   \\ 
J2043+2740 & J2043+2740 & 0.23 & 5.6e+34 & 1.8 & --- & {15.}$^{d}$ &    &  X &   &   &   &   \\ 
J0855$-$4644 & J0855$-$4644 & 0.22 & 1.1e+36 & 3.9 & 0.20 & --- &    &    &   &   &   &   \\ 
J0218+4232 & J0218+4232 & 0.22 & 2.4e+35 & 2.7 & 0.90 & 35. &    &  X & 3EG J0222+4253 & 1.03 &   &   \\ 
J1739$-$3023 & J1739$-$3023 & 0.20 & 3.0e+35 & 2.9 & 1.00 & --- &    &    & 3EG J1744$-$3011 (*) & 1.10 &   &   \\ 
J1831$-$0952 & J1831$-$0952 & 0.20 & 1.1e+36 & 4.0 & 0.33 & --- &    &    &   &   &   &   \\ 
B1957+20 & J1959+2048 & 0.20 & 1.6e+35 & 2.5 & 0.40 & 20. &    &  np &   &   &   & G59.2$-$4.7 \\ 
J1105$-$6107 & J1105$-$6107 & 0.20 & 2.5e+36 & 5.0 & 0.75 & --- &    &  np & 3EG J1102$-$6103 & 0.86 &   & MSH 11$-$62 \\ 
B1821$-$24 & J1824$-$2452 & 0.19 & 2.2e+36 & 4.9 & 0.18 & 40. & M28  &  X &   &   &   &   \\ 
B1853+01 & J1856+0113 & 0.19 & 4.3e+35 & 3.3 & 0.19 & 3.40 &    &    & 3EG J1856+0114 & 0.05 &   & G34.7$-$0.4, W44, 3C 392 \\ 
B1757$-$24 & J1801$-$2451 & 0.18 & 2.6e+36 & 5.2 & 0.85 & 7.80 &    &  np & 3EG J1800$-$2338 & 1.26 &   & G5.27$-$0.9,G5.4-1.2? \\ 
B0611+22 & J0614+2229 & 0.18 & 6.2e+34 & 2.1 & 2.20 & 29. &    &    & 3EG J0617+2238 & 0.69 &   &   \\ 
B1719$-$37 & J1722$-$3712 & 0.16 & 3.3e+34 & 1.9 & 3.20 & 25. &    &    &   &   &   &   \\ 
J1835$-$1106 & J1835$-$1106 & 0.16 & 1.8e+35 & 2.8 & 2.20 & 30. &    &    &   &   &   &   \\ 
B0540+23 & J0543+2329 & 0.15 & 4.1e+34 & 2.1 & 9.00 & 29. &    &    &   &   &   &   \\ 
J1913+0904 & J1913+0904 & 0.14 & 1.6e+35 & 3.0 & 0.07 & --- &    &    &   &   &   &   \\ 
J0857$-$4424 & J0857$-$4424 & 0.13 & 2.6e+34 & 1.9 & 0.88 & 12. &    &    &   &   &   &   \\ 
J0729$-$1448 & J0729$-$1448 & 0.13 & 2.8e+35 & 3.5 & 0.70 & --- &    &    &   &   &   &   \\ 
B1737$-$30 & J1740$-$3015 & 0.12 & 8.2e+34 & 2.7 & 6.40 & 25. &    &    & 3EG J1744$-$3011 (*) & 0.86 &   &   \\ 
J1928+1746 & J1928+1746 & 0.11 & 1.6e+36 & 5.8 & 0.25 & --- &    &    & 3EG J1928+1733 & 0.29 &   &   \\ 
J1015$-$5719 & J1015$-$5719 & 0.11 & 8.3e+35 & 5.1 & 0.90 & --- &    &    & 3EG J1014$-$5705 & 0.47 &   &   \\ 
B1830$-$08 & J1833$-$0827 & 0.11 & 5.8e+35 & 4.7 & 3.60 & --- &    &    &   &   & HESS J1834$-$087 &   \\ 
J1837$-$0604 & J1837$-$0604 & 0.11 & 2.0e+36 & 6.4 & 0.70 & --- &    &    & 3EG J1837$-$0606 (*) & 0.18 &   &   \\ 
J1740$-$5340A & J1740$-$5340A & 0.10 & 1.4e+35 & 3.4 & { 1.}$^{e}$ & --- & NGC6397  &    &   &   &   &   \\ 
B1449$-$64 & J1453$-$6413 & 0.10 & 1.9e+34 & 2.1 & 14. & 230. &    &    &   &   &   &   \\ 
J1637$-$4642 & J1637$-$4642 & 0.099 & 6.4e+35 & 5.1 & 0.78 & --- &    &    & 3EG J1639$-$4702 & 0.55 &   &   \\ 
J0631+1036 & J0631+1036 & 0.098 & 1.7e+35 & 3.7 & 0.80 & 1.50 &    &  X &   &   &   &   \\ 
J1702$-$4310 & J1702$-$4310 & 0.096 & 6.3e+35 & 5.1 & 0.72 & --- &    &    &   &   &   &   \\ 
J1301$-$6305 & J1301$-$6305 & 0.094 & 1.7e+36 & 6.7 & 0.46 & --- &    &    &   &   & HESS J1301$-$631 &   \\ 
J1828$-$1101 & J1828$-$1101 & 0.092 & 1.6e+36 & 6.6 & 2.90 & --- &    &    &   &   &   &   \\ 
B1620$-$26 & J1623$-$2631 & 0.091 & 2.0e+34 & 2.2 & 1.60 & 15. & M4  &    & 3EG J1626$-$2519 & 1.35 &   &   \\ 
B1634$-$45 & J1637$-$4553 & 0.087 & 7.5e+34 & 3.2 & 1.10 & 15. &    &    & 3EG J1639$-$4702 & 1.17 &   &   \\ 
J1702$-$4128 & J1702$-$4128 & 0.082 & 3.4e+35 & 4.8 & 1.10 & --- &    &    &   &   & HESS J1702$-$420 &   \\ 
J1705$-$3950 & J1705$-$3950 & 0.081 & 7.4e+34 & 3.3 & 1.50 & --- &    &    &   &   &   &   \\ 
J1016$-$5857 & J1016$-$5857 & 0.080 & 2.6e+36 & 8.0 & 0.46 & --- &    &    & 3EG J1013$-$5915 (*) & 0.89 &   & G284.3$-$1.8 \\ 
J0901$-$4624 & J0901$-$4624 & 0.080 & 4.0e+34 & 2.8 & 0.46 & --- &    &    &   &   &   &   \\ 
B2334+61 & J2337+6151 & 0.080 & 6.2e+34 & 3.1 & 1.40 & 10. &    &  np &   &   &   &   \\ 
B1317$-$53 & J1320$-$5359 & 0.076 & 1.7e+34 & 2.3 & --- & 18. &    &    & 3EG J1316$-$5244 & 1.75 &   &   \\ 
J1841$-$0345 & J1841$-$0345 & 0.073 & 2.7e+35 & 4.8 & 1.40 & --- &    &    & 3EG J1837$-$0423 & 1.29 &   &   \\ 
J1830$-$0131 & J1830$-$0131 & 0.069 & 2.3e+34 & 2.6 & 0.35 & --- &    &    &   &   &   &   \\ 
J1119$-$6127 & J1119$-$6127 & 0.068 & 2.3e+36 & 8.4 & 0.80 & --- &    &  np &   &   &   & G292.2$-$0.5 \\ 
J1549$-$4848 & J1549$-$4848 & 0.068 & 2.3e+34 & 2.7 & 0.47 & 17. &    &    &   &   &   &   \\ 
J1816$-$0755 & J1816$-$0755 & 0.065 & 2.5e+34 & 2.8 & 0.17 & --- &    &    &   &   &   &   \\ 
J1857+0143 & J1857+0143 & 0.064 & 4.5e+35 & 5.8 & 0.74 & --- &    &    & 3EG J1856+0114 & 0.63 & HESS J1858+020 &   \\ 
B1001$-$47 & J1003$-$4747 & 0.064 & 3.0e+34 & 2.9 & --- & 6.00 &    &    &   &   &   &   \\ 
B1610$-$50 & J1614$-$5048 & 0.064 & 1.6e+36 & 7.9 & 2.40 & --- &    &    &   &   &   &   \\ 
B1828$-$11 & J1830$-$1059 & 0.060 & 3.6e+34 & 3.2 & 1.40 & 2.10 &    &    &   &   &   &   \\ 
J1648$-$4611 & J1648$-$4611 & 0.059 & 2.1e+35 & 5.0 & 0.58 & --- &    &    & 3EG J1655$-$4554 & 1.68 &   &   \\ 
B1643$-$43 & J1646$-$4346 & 0.057 & 3.6e+35 & 5.8 & 0.98 & --- &    &    &   &   &   & G341.2+0.9 \\ 
J1906+0746 & J1906+0746 & 0.057 & 2.7e+35 & 5.4 & 0.55 & 0.90 &    &    &   &   &   &   \\ 
B0136+57 & J0139+5814 & 0.055 & 2.1e+34 & 2.9 & 4.60 & 28. &    &    &   &   &   &   \\ 
J1738$-$2955 & J1738$-$2955 & 0.050 & 3.7e+34 & 3.5 & 0.29 & --- &    &    & 3EG J1736$-$2908 (*) & 1.07 &   &   \\ 
B1730$-$37 & J1733$-$3716 & 0.050 & 1.5e+34 & 2.8 & 3.40 & --- &    &    &   &   &   &   \\ 
B0021$-$72F & J0024$-$7204F & 0.049 & 1.4e+35 & 4.9 & { 0.15}$^{f}$ & --- & 47Tuc  &    &   &   &   &   \\ 
J1723$-$3659 & J1723$-$3659 & 0.049 & 3.8e+34 & 3.5 & 1.50 & --- &    &    &   &   &   &   \\ 
J1715$-$3903 & J1715$-$3903 & 0.049 & 6.9e+34 & 4.1 & 0.46 & --- &    &    & 3EG J1714$-$3857 & 0.33 &   &   \\ 
J1601$-$5335 & J1601$-$5335 & 0.048 & 1.0e+35 & 4.5 & 0.22 & --- &    &    &   &   &   &   \\ 
J1514$-$5925 & J1514$-$5925 & 0.048 & 3.5e+34 & 3.5 & 0.27 & --- &    &    &   &   & HESS J1514$-$591 &   \\ 
B1937+21 & J1939+2134 & 0.048 & 1.1e+36 & 8.3 & 10. & 240. &    &  X &   &   &   &   \\ 
B1820$-$30A & J1823$-$3021A & 0.046 & 8.3e+35 & 7.9 & 0.72 & 16. & NGC6624  &    &   &   &   &   \\ 
J1828$-$1057 & J1828$-$1057 & 0.046 & 5.5e+34 & 4.0 & 0.23 & --- &    &    &   &   &   &   \\ 
J0905$-$5127 & J0905$-$5127 & 0.045 & 2.4e+34 & 3.3 & 1.10 & 12. &    &    &   &   &   &   \\ 
J1112$-$6103 & J1112$-$6103 & 0.045 & 4.5e+36 & 12.2 & 1.40 & --- &    &    &   &   &   &   \\ 
B1221$-$63 & J1224$-$6407 & 0.044 & 1.9e+34 & 3.1 & 3.90 & 48. &    &    &   &   &   &   \\ 
B1727$-$47 & J1731$-$4744 & 0.042 & 1.1e+34 & 2.8 & 12. & 190. &    &    &   &   &   &   \\ 
B1356$-$60 & J1359$-$6038 & 0.041 & 1.2e+35 & 5.2 & 7.60 & 105. &    &    &   &   &   &   \\ 
J1921+0812 & J1921+0812 & 0.040 & 2.3e+34 & 3.5 & 0.66 & --- &    &    &   &   &   &   \\ 
B1915+13 & J1917+1353 & 0.039 & 3.8e+34 & 4.0 & 1.90 & 43. &    &    &   &   &   &   \\ 
B0021$-$72E & J0024$-$7204E & 0.039 & 8.8e+34 & 4.9 & { 0.21}$^{f}$ & --- & 47Tuc  &    &   &   &   &   \\ 
J1838$-$0549 & J1838$-$0549 & 0.039 & 1.0e+35 & 5.1 & 0.29 & --- &    &    & 3EG J1837$-$0606 (*) & 0.50 & HESS J1841$-$055 &   \\ 
J1548$-$5607 & J1548$-$5607 & 0.039 & 8.5e+34 & 4.9 & 1.00 & --- &    &    &   &   &   &   \\ 
J1835$-$0944 & J1835$-$0944 & 0.039 & 5.6e+34 & 4.4 & 0.41 & --- &    &    &   &   &   &   \\ 
 J2021+3651  & J2021+3651 & 0.038 & 3.4e+36 & 12.4 & 0.10 & --- &    &  X & 3EG J2021+3716 (*) & 0.41 & MGRO J2019+37 & G75.2+0.1 \\ 
B1535$-$56 & J1539$-$5626 & 0.037 & 1.3e+34 & 3.1 & 4.60 & --- &    &    &   &   &   &   \\ 
J1638$-$4608 & J1638$-$4608 & 0.036 & 9.4e+34 & 5.2 & 0.33 & --- &    &    & 3EG J1639$-$4702 & 0.91 &   &   \\ 
J1910$-$5959D & J1910$-$5959D & 0.036 & 5.2e+34 & 4.5 & 0.05 & --- & NGC6752  &    &   &   &   &   \\ 
J1841$-$0524 & J1841$-$0524 & 0.035 & 1.0e+35 & 5.3 & 0.20 & --- &    &    & 3EG J1837$-$0606 (*) & 1.39 & HESS J1841$-$055 &   \\ 
J0024$-$7204O & J0024$-$7204O & 0.033 & 6.5e+34 & 4.9 & { 0.10}$^{f}$ & --- & 47Tuc  &    &   &   &   &   \\ 
B1754$-$24 & J1757$-$2421 & 0.033 & 4.0e+34 & 4.4 & 3.90 & 20. &    &    & 3EG J1800$-$2338 & 0.97 &   &   \\ 
J1452$-$5851 & J1452$-$5851 & 0.032 & 3.5e+34 & 4.3 & 0.24 & --- &    &    &   &   &   &   \\ 
J1541$-$5535 & J1541$-$5535 & 0.032 & 1.1e+35 & 5.7 & 0.22 & --- &    &    &   &   &   &   \\ 
J1643$-$4505 & J1643$-$4505 & 0.031 & 9.4e+34 & 5.6 & 0.28 & --- &    &    &   &   &   &   \\ 
B1607$-$52 & J1611$-$5209 & 0.031 & 3.4e+34 & 4.3 & 1.20 & --- &    &    &   &   &   &   \\ 
B1338$-$62 & J1341$-$6220 & 0.030 & 1.4e+36 & 11.1 & 1.90 & --- &    &  X &   &   &   & G308.8$-$0.1 \\ 
J1907+0918 & J1907+0918 & 0.029 & 3.2e+35 & 7.8 & 0.29 & 0.40 &    &    &   &   &   &   \\ 
J1016$-$5819 & J1016$-$5819 & 0.029 & 4.1e+34 & 4.7 & 0.31 & --- &    &    & 3EG J1013$-$5915 (*) & 1.23 &   &   \\ 
J0537$-$6910 & J0537$-$6910 & 0.029 & 4.9e+38 & 49.4 & --- & --- &  LMC &  X & 3EG J0533$-$6916 & 1.20 &   & G279.6$-$31.7, N 157B \\ 
B1930+22 & J1932+2220 & 0.028 & 7.5e+35 & 9.8 & 1.20 & 7.80 &    &    &   &   &   &   \\ 
J1853$-$0004 & J1853$-$0004 & 0.028 & 2.1e+35 & 7.2 & 0.87 & --- &    &    & 3EG J1856+0114 & 1.46 &   &   \\ 
J0024$-$7204U & J0024$-$7204U & 0.028 & 4.6e+34 & 4.9 & { 0.06}$^{f}$ & --- & 47Tuc  &    &   &   &   &   \\ 
J1019$-$5749 & J1019$-$5749 & 0.028 & 1.8e+35 & 6.9 & 0.80 & --- &    &    & 3EG J1014$-$5705 (*) & 1.64 &   &   \\ 
B1556$-$57 & J1600$-$5751 & 0.027 & 1.1e+34 & 3.5 & 1.40 & 20. &    &    &   &   &   &   \\ 
J1841+0130 & J1841+0130 & 0.027 & 1.2e+34 & 3.6 & 0.06 & --- &    &    &   &   &   &   \\ 
J1543$-$5459 & J1543$-$5459 & 0.026 & 3.8e+34 & 4.8 & 0.62 & --- &    &    &   &   &   &   \\ 
J0954$-$5430 & J0954$-$5430 & 0.026 & 1.6e+34 & 3.9 & 0.36 & --- &    &    &   &   &   &   \\ 
J1737$-$3137 & J1737$-$3137 & 0.026 & 6.0e+34 & 5.5 & 0.80 & --- &    &    & 3EG J1734$-$3232 & 1.19 &   &   \\ 
J1650$-$4921 & J1650$-$4921 & 0.025 & 1.9e+34 & 4.1 & 0.16 & --- &    &    &   &   &   &   \\ 
J1815$-$1738 & J1815$-$1738 & 0.025 & 3.9e+35 & 8.8 & 0.25 & --- &    &    &   &   & HESS J1813$-$178 &   \\ 
B1822$-$14 & J1825$-$1446 & 0.025 & 4.1e+34 & 5.1 & 2.60 & --- &    &    & 3EG J1824$-$1514 (*) & 0.52 & HESS J1826$-$148  &   \\ 
B1821$-$19 & J1824$-$1945 & 0.024 & 3.0e+34 & 4.7 & 4.90 & 71. &    &    &   &   &   &   \\ 
J1853+0056 & J1853+0056 & 0.024 & 4.0e+34 & 5.1 & 0.21 & --- &    &    & 3EG J1856+0114 & 0.68 &   &   \\ 
J1115$-$6052 & J1115$-$6052 & 0.023 & 1.6e+34 & 4.1 & 0.38 & --- &    &    &   &   &   &   \\ 
J1903+0925 & J1903+0925 & 0.023 & 3.2e+34 & 4.9 & 0.20 & --- &    &    &   &   &   &   \\ 
J1413$-$6141 & J1413$-$6141 & 0.023 & 5.6e+35 & 10.1 & 0.61 & --- &    &    & 3EG J1410$-$6147 & 0.80 &   &   \\ 
J1756$-$2225 & J1756$-$2225 & 0.023 & 3.1e+34 & 5.0 & 0.25 & --- &    &    & 3EG J1800$-$2338 & 1.50 &   &   \\ 
J1406$-$6121 & J1406$-$6121 & 0.022 & 2.2e+35 & 8.2 & 0.36 & --- &    &    & 3EG J1410$-$6147 & 0.90 &   &   \\ 
J0024$-$7204T & J0024$-$7204T & 0.021 & 2.7e+34 & 4.9 & --- & --- & 47Tuc  &    &   &   &   &   \\ 
B1718$-$35 & J1721$-$3532 & 0.021 & 4.5e+34 & 5.6 & 11. & --- &    &    &   &   &   &   \\ 
B1508$-$57 & J1512$-$5759 & 0.021 & 1.3e+35 & 7.3 & 6.00 & --- &    &    &   &   &   &   \\ 
B1832$-$06 & J1835$-$0643 & 0.019 & 5.6e+34 & 6.2 & 1.30 & --- &    &    & 3EG J1837$-$0606 & 0.78 &   &   \\ 
B1838$-$04 & J1841$-$0425 & 0.019 & 3.9e+34 & 5.7 & 2.60 & 2.60 &    &    & 3EG J1837$-$0423 (*) & 1.02 &   &   \\ 
J1538$-$5551 & J1538$-$5551 & 0.019 & 1.1e+35 & 7.5 & 0.25 & --- &    &    &   &   &   &   \\ 
J0024$-$7204Q & J0024$-$7204Q & 0.018 & 2.0e+34 & 4.9 & { 0.05}$^{f}$ & --- & 47Tuc  &    &   &   &   &   \\ 
J1138$-$6207 & J1138$-$6207 & 0.018 & 3.0e+35 & 9.7 & 0.49 & --- &    &    &   &   &   &   \\ 
J1156$-$5707 & J1156$-$5707 & 0.018 & 4.3e+34 & 6.0 & 0.19 & --- &    &    &   &   &   &   \\ 
J1734$-$3333 & J1734$-$3333 & 0.018 & 5.6e+34 & 6.5 & 0.50 & --- &    &    & 3EG J1734$-$3232 & 1.03 &   &   \\ 
J1412$-$6145 & J1412$-$6145 & 0.018 & 1.2e+35 & 7.8 & 0.47 & --- &    &    & 3EG J1410$-$6147 & 0.53 &   &   \\ 
J1743$-$3153 & J1743$-$3153 & 0.017 & 5.8e+34 & 6.6 & 0.50 & --- &    &    & 3EG J1744$-$3011 & 1.71 &   &   \\ 
J1632$-$4757 & J1632$-$4757 & 0.017 & 5.0e+34 & 6.4 & 0.30 & --- &    &    & 3EG J1639$-$4702 & 1.92 & HESS J1632$-$478 &   \\ 
J1123$-$6259 & J1123$-$6259 & 0.017 & 1.0e+34 & 4.3 & 0.56 & 11. &    &    &   &   &   &   \\ 
J1909+0912 & J1909+0912 & 0.017 & 1.3e+35 & 8.2 & 0.35 & --- &    &    &   &   &   &   \\ 
J1650$-$4502 & J1650$-$4502 & 0.017 & 1.1e+34 & 4.4 & 0.35 & --- &    &    & 3EG J1655$-$4554 & 1.41 &   &   \\ 
J1638$-$4417 & J1638$-$4417 & 0.016 & 3.9e+34 & 6.2 & 0.21 & --- &    &    &   &   &   &   \\ 
B0540$-$69 & J0540$-$6919 & 0.016 & 1.5e+38 & 49.4 & 0.02 & --- &  LMC & OX & 3EG J0533$-$6916 & 1.80 &   & G279.7$-$31.5, N158A \\ 
J1834$-$0731 & J1834$-$0731 & 0.015 & 1.7e+34 & 5.1 & 1.00 & --- &    &    & 3EG J1837$-$0606 & 1.57 &   &   \\ 
J1052$-$5954 & J1052$-$5954 & 0.015 & 1.3e+35 & 8.5 & 0.15 & --- &    &    & 3EG J1048$-$5840 & 1.70 &   &   \\ 
B2148+52 & J2150+5247 & 0.015 & 1.1e+34 & 4.6 & 2.00 & 16. &    &    &   &   &   &   \\ 
J1649$-$4653 & J1649$-$4653 & 0.015 & 1.1e+34 & 4.7 & 0.31 & --- &    &    & 3EG J1655$-$4554 & 1.71 &   &   \\ 
J1551$-$5310 & J1551$-$5310 & 0.015 & 8.3e+34 & 7.8 & 0.54 & --- &    &    &   &   &   &   \\ 
J1843$-$0702 & J1843$-$0702 & 0.015 & 1.2e+34 & 4.8 & 0.17 & --- &    &    & 3EG J1837$-$0606 & 1.85 &   &   \\ 
J1907+0919 & J1907+0919 & 0.014 & 2.2e+34 & 5.8 & --- & --- &    &    &   &   &   &   \\ 
J1349$-$6130 & J1349$-$6130 & 0.014 & 1.2e+34 & 5.0 & 0.58 & --- &    &    &   &   &   &   \\ 
J1913+0832 & J1913+0832 & 0.014 & 7.4e+34 & 7.9 & 0.60 & --- &    &    &   &   &   &   \\ 
J1838$-$0453 & J1838$-$0453 & 0.013 & 8.3e+34 & 8.1 & 0.33 & --- &    &    & 3EG J1837$-$0423 (*) & 0.59 &   &   \\ 
J1627$-$4706 & J1627$-$4706 & 0.013 & 2.5e+34 & 6.1 & 0.10 & --- &    &    &   &   &   &   \\ 
J1837$-$0559 & J1837$-$0559 & 0.013 & 1.6e+34 & 5.4 & 0.50 & --- &    &    & 3EG J1837$-$0606 (*) & 0.15 & HESS J1841$-$055 &   \\ 
J1248$-$6344 & J1248$-$6344 & 0.013 & 8.6e+34 & 8.3 & 0.12 & --- &    &    &   &   &   &   \\ 
J1845$-$0743 & J1845$-$0743 & 0.013 & 1.3e+34 & 5.2 & 2.70 & --- &    &    &   &   &   &   \\ 
J1839$-$0905 & J1839$-$0905 & 0.012 & 1.4e+34 & 5.4 & 0.16 & --- &    &    &   &   &   &   \\ 
J1845$-$0316 & J1845$-$0316 & 0.012 & 3.9e+34 & 7.0 & 0.35 & --- &    &    &   &   & HESS J1846$-$029 &   \\ 
J1801$-$2154 & J1801$-$2154 & 0.012 & 1.2e+34 & 5.3 & 0.18 & --- &    &    & 3EG J1800$-$2338 & 1.75 &   &   \\ 
J1853+0545 & J1853+0545 & 0.012 & 1.2e+34 & 5.3 & 1.60 & --- &    &    &   &   &   &   \\ 
J1907+0731 & J1907+0731 & 0.011 & 1.5e+34 & 5.7 & 0.35 & --- &    &    &   &   &   &   \\ 
B1557$-$50 & J1600$-$5044 & 0.011 & 2.8e+34 & 6.7 & 17. & --- &    &    &   &   &   &   \\ 
J1755$-$2534 & J1755$-$2534 & 0.011 & 3.5e+34 & 7.1 & 0.17 & --- &    &    &   &   &   &   \\ 
J1452$-$6036 & J1452$-$6036 & 0.011 & 1.5e+34 & 5.8 & 1.40 & --- &    &    &   &   &   &   \\ 
J1839$-$0321 & J1839$-$0321 & 0.011 & 3.6e+34 & 7.2 & 0.27 & --- &    &    & 3EG J1837$-$0423 & 1.22 &   &   \\ 
J1632$-$4818 & J1632$-$4818 & 0.011 & 4.8e+34 & 7.8 & 0.39 & --- &    &    &   &   & HESS J1632$-$478 &   \\ 
B1841$-$05 & J1844$-$0538 & 0.011 & 2.3e+34 & 6.5 & 2.20 & --- &    &    & 3EG J1837$-$0606 & 1.83 &   &   \\ 
J1550$-$5418 & J1550$-$5418 & 0.011 & 1.0e+35 & 9.6 & 3.30 & --- &    &    &   &   &   &   \\ 
B2000+32 & J2002+3217 & 0.010 & 1.2e+34 & 5.7 & 1.20 & 5.50 &    &    &   &   &   &   \\ 
J1907+0345 & J1907+0345 & 0.0094 & 2.3e+34 & 7.2 & 0.17 & --- &    &    &   &   &   &   \\ 
J1842$-$0905 & J1842$-$0905 & 0.0091 & 1.0e+34 & 5.9 & 0.81 & --- &    &    &   &   &   &   \\ 
J1946+2611 & J1946+2611 & 0.0089 & 1.1e+34 & 6.1 & --- & 1.50 &    &    &   &   &   &   \\ 
J1726$-$3530 & J1726$-$3530 & 0.0084 & 3.5e+34 & 8.4 & 0.30 & --- &    &    &   &   &   &   \\ 
B1636$-$47 & J1640$-$4715 & 0.0083 & 1.2e+34 & 6.5 & 1.20 & --- &    &    & 3EG J1639$-$4702 & 0.38 &   &   \\ 
J1904+0800 & J1904+0800 & 0.0082 & 3.7e+34 & 8.6 & 0.36 & --- &    &    &   &   &   &   \\ 
J1820$-$1529 & J1820$-$1529 & 0.0080 & 4.0e+34 & 8.9 & 0.61 & --- &    &    & 3EG J1824$-$1514 & 0.87 &   &   \\ 
B2011+38 & J2013+3845 & 0.0076 & 2.9e+34 & 8.4 & 6.40 & 26. &    &    & 3EG J2016+3657 & 1.95 &   &   \\ 
J1908+0909 & J1908+0909 & 0.0075 & 3.6e+34 & 9.0 & 0.22 & --- &    &    &   &   &   &   \\ 
B1855+02 & J1857+0212 & 0.0074 & 2.2e+34 & 8.0 & 1.60 & --- &    &    & 3EG J1856+0114 & 1.07 & HESS J1858+020 &   \\ 
J1903+0601 & J1903+0601 & 0.0073 & 1.5e+34 & 7.2 & 0.26 & --- &    &    & 3EG J1903+0550 & 0.21 &   &   \\ 
J1515$-$5720 & J1515$-$5720 & 0.0072 & 1.0e+34 & 6.6 & 0.20 & --- &    &    &   &   &   &   \\ 
J1853+0011 & J1853+0011 & 0.0070 & 2.1e+34 & 8.1 & 0.30 & --- &    &    & 3EG J1856+0114 & 1.21 &   &   \\ 
J1342+2822B & J1342+2822B & 0.0068 & 5.4e+34 & 10.4 & 0.01 & --- & M3  &    &   &   &   &   \\ 
J1806$-$2125 & J1806$-$2125 & 0.0068 & 4.3e+34 & 9.8 & 1.10 & --- &    &    &   &   &   &   \\ 
J1626$-$4807 & J1626$-$4807 & 0.0066 & 2.7e+34 & 8.9 & 0.37 & --- &    &    &   &   &   &   \\ 
J1020$-$6026 & J1020$-$6026 & 0.0065 & 9.6e+34 & 12.3 & 0.14 & --- &    &    &   &   &   &   \\ 
J1305$-$6203 & J1305$-$6203 & 0.0055 & 1.6e+34 & 8.5 & 0.62 & --- &    &    & 3EG J1308$-$6112 & 1.08 &   &   \\ 
J1843$-$0355 & J1843$-$0355 & 0.0055 & 1.8e+34 & 8.8 & 0.80 & --- &    &    & 3EG J1837$-$0423 & 1.59 &   &   \\ 
J1735$-$3258 & J1735$-$3258 & 0.0054 & 2.4e+34 & 9.6 & 0.46 & --- &    &    & 3EG J1734$-$3232 & 0.66 &   &   \\ 
B2127+11E & J2129+1210E & 0.0050 & 7.0e+34 & 12.9 & --- & 0.20 & M15  &    &   &   &   &   \\ 
B1758$-$23 & J1801$-$2304 & 0.0050 & 6.2e+34 & 12.6 & 2.20 & --- &    &    & 3EG J1800$-$2338 (*) & 0.65 &   &   \\ 
J1043$-$6116 & J1043$-$6116 & 0.0046 & 1.7e+34 & 9.5 & 0.91 & --- &    &    &   &   &   &   \\ 
J1908+0839 & J1908+0839 & 0.0045 & 1.5e+34 & 9.3 & 0.49 & --- &    &    &   &   &   &   \\ 
J1808$-$2024 & J1808$-$2024 & 0.0041 & 5.0e+34 & 13.1 & --- & --- &    &    &   &   &   &   \\ 
J1812$-$1910 & J1812$-$1910 & 0.0035 & 1.9e+34 & 11.2 & 0.22 & --- &    &    &   &   &   &   \\ 
J1327$-$6400 & J1327$-$6400 & 0.0031 & 5.6e+34 & 15.5 & 0.36 & --- &    &    &   &   &   &   \\ 
B2127+11F & J2129+1210F & 0.0026 & 1.9e+34 & 12.9 & --- & 0.10 & M15  &    &   &   &   &   \\ 
J1524$-$5706 & J1524$-$5706 & 0.0024 & 1.0e+34 & 11.4 & 0.41 & --- &    &    &   &   &   &   \\ 
J1216$-$6223 & J1216$-$6223 & 0.0013 & 1.3e+34 & 16.6 & 0.15 & --- &    &    &   &   &   &   \\ 
J0535$-$6935 & J0535$-$6935 & 0.00031 & 5.6e+34 & 49.4 & 0.05 & --- &  LMC &    & 3EG J0533$-$6916 & 0.59 &   &   \\ 
B0456$-$69 & J0455$-$6951 & 0.00014 & 1.2e+34 & 49.4 & --- & 0.60 &  LMC &    &   &   &   &   \\ 
\end{supertabular}
%\end{scriptsize}
\end{tiny}
\end{center}
\label{tab1}
\end{landscape}


==> part2/conclusion.tex <==
\chapter*{Conclusion} 

[Conclusion de la partie 2]


==> part3/conclusion.tex <==
\chapter*{Conclusion} 

[Conclusion de la partie 2]


==> part3/introduction.tex <==
\chapter*{Introduction} 

Les chapitres suivants présentent la découverte $\gamma$ de trois pulsars radio individuels, PSRs J0205+6449, J2229+6114, et J1048$-$5832, ainsi que le premier catalogue de pulsars du télescope \textit{Fermi}. Les résultats sont basés sur les analyses temporelles et spectrales exposées au chapitre \ref{chap:analyse}. \\

Nous analyserons les courbes de lumière $\gamma$ en fonction de l'énergie et les spectres en énergies des différents objets. , et nous discuterons de la luminosité, de l'efficacité $\gamma$, et de la géométrie de leur émission. 


==> tableaux/CharacParTable.tex <==
\begin{scriptsize}
\begin{tabular}{llrrrrrrrr}
\hline 
\hline
PSR & Type, & $l$ \ \ \ & $b$ \ \ & P \ \ & \.{P} \ \ \ & age $\tau_{{\rm c}}$ & $\dot E \ \ \ \ \ \ \ $ & B$_{LC}$ & $S_{1400}$  \\
    & \textit{Ref.} & ($^\circ$) \ & ($^\circ$) \ & (ms) & ($10^{-15}$) & (kyr) & ($10^{34}$ erg s$^{-1}$) & (kG) & (mJy) \\
\hline
\vspace{0.4mm}
J0007$+$7303	 &	g  $^{a,b}$ &  119.7   &  10.5  &	 316   &	361		&	  14		    &		   45.2    &    	 3.1     &	$^1\,<0.1$ \ 		\\
J0030$+$0451	 &	m  $^{c,d}$ &	 113.1   & $-$57.6   &	 4.9  &  10 $\times 10^{-6}$  &	7.7$\times 10^{6}$ &	 0.3   &	17.8    &		  0.6 \ 		\\
J0205$+$6449	 &	r  $^e$     &	 130.7   &	 3.1   &   65.7    & 194	&	    5	   &	 2700 &	115.9  &	0.04			\\
J0218$+$4232	 & mb $^d$     &	139.5   &	 $-$17.5   &	       2.3    &  77$\times 10^{-6}$   &	0.5$\times 10^{6}$ &	24 &	313.1   &		  0.9 \ 		\\
J0248$+$6021	 & r  $^f$     & 137.0   & v0.4     &	   217    &	  55.1	    &	  63		    &		  21 &	3.1	  &		  9	\\
J0357$+$32	   & g  $^b$     & 162.7   &	  $-$16.0   &	   444   &	  12.0	&	590		    &	  0.5     &		0.2	  &		...			\\
J0437$-$4715	 & mb $^d$     &	253.4   &	 $-$42.0   &	 5.8    &  14$\times 10^{-6}$   &	6.6$\times 10^{6}$ &  0.3  &	 	13.7    &	   140 	\\
J0534$+$2200	 & r  $^h$     & 184.6   & $-$5.8    &	 33.1    &	423	&	     1	  &	    46100 &	950.0   &            14	\\
J0613$-$0200	 & mb $^d$     &  210.4   &	 $-$9.3    &	 3.1    &    9n$\times 10^{-6}$    &	5.3$\times 10^{6}$ &  1.3    & 54.3    &	1.4 \   	\\
J0631$+$1036	 & r  $^i$     & 201.2   &	  0.5     &	   288    &	105	&	  44		    &		  17.3    &	  	2.1	  &		  0.8 \      	\\
J0633$+$0632   & g  $^b$     & 205.0   &	 $-$1.0    &	   297   &	  79.5   &	  59	 &	 11.9    &	  	1.7	  &	   $^2\,<0.2$ \ 	\\
J0633$+$1746	 & g  $^h$     & 195.1   &	  4.3     &	   237   &	  11.0	&	340 	  &		  3.3    &	 	1.1	  &	$<1$ \  \ 	\\
J0659$+$1414	 & r  $^i$     &	 201.1   &	8.3     &	   385  &	  55.0		       &	110 		    &		    3.8    &		0.7	  &		  3.7 \      	\\
J0742$-$2822	 & r  $^i$     &	 243.8   &   $-$2.4  &	   167   &	  16.8 &	160    &		  14.3    &	  	3.3	  &  15     \\
J0751$+$1807	 & mb $^d$     &	  202.7   &	    21.1  &	 3.5    &	6.2$\times 10^{-6}$    &	8.0$\times 10^{6}$ &	  0.6  &		32.3  &  3.2 \  	\\
J0835$-$4510	 & r  $^k$     & 263.6   &	       $-$2.8    & 89.3    &		124	&	  11		    &		688 &	43.4    &		  1100   \\	
J1028$-$5819	 & r  $^l$     & 285.1   &	 $-$0.5    &	     91.4    &	 16.1	  &	  90   &		  83.2    &	  	14.6    &		  0.36 	\\
J1048$-$5832	 & r  $^m$     & 287.4   &	  0.6  & 124   &	  96.  &	  20  &		201 &	16.8    &		  6.5 \      	\\
J1057$-$5226	 & r  $^n$     &   286.0   &	     6.6     &	  197   &	    5.8	  &	540  &   3.0    &	  	1.3	  &		  11  \\
J1124$-$5916	 & r	       &	  292.0   &	  1.8     &	 135  &	747	&	    3		    &	       1190 &	37.3    &		  0.08     		\\
J1418$-$6058	 & g  $^b$     & 313.3   &	 0.1     &	   111   &	170	&	  10		    &		495 &	29.4    &	  $^{2,3}\,<0.06$  	\\
J1420$-$6048	 & r  $^i$     &  313.5   &	 0.2     &	   68.2    &	83.2	  &	  13  &	 1000  &	69.1    &		  0.9 \   	\\
J1459$-$60	   & g  $^b$     & 317.9   & $-$1.8    & 103  &	  25.5 &	  64	&		  91.9    &	  	13.6    &	    $^2\,<0.2$ \ 	\\
J1509$-$5850	 & r  $^i$     & 320.0   & $-$0.6    &	  88.9    &	   9.2	&	150 	  & 51.5    &		11.8    &	  0.15    		\\
J1614$-$2230	 & mb $^d$     &	352.5   &	  20.3    &	  3.2    &  4$\times 10^{-6}$ &	1.2$\times 10^{	6}$ &  0.5  &	 	33.7    &	 ...	  	\\
J1709$-$4429	 & r  $^n$     &	343.1   &	 $-$2.7    &	   102  &	  93.0	 &	  18	  &		341&	26.4    &		  7.3 \   	\\
J1718$-$3825	 & r  $^i$     &	349.0  &	  $-$0.4    &	   74.7  &	  	  13.2	  &	  90	  &		125 &	21.9    &		  1.3 \      	\\
J1732$-$31	   & g  $^b$     &	356.2   &	 0.9     & 197   &	  26.1   &	120		    &		  13.6    &	  	2.7	  &	    $^2\,<0.2$ \ 	\\
J1741$-$2054	 & g  $^{b,t}$ &	6.4  &	4.6  &414 &	  16.9		       &	390		    &		    0.9     &	  	0.3	  & 	    $^2\,0.16$    		\\
J1744$-$1134	 & m  $^d$     &	14.8    &	 9.2     & 4.1    &  7$\times 10^{-6}$   &	 9$\times 10^{6}$ &	  0.4    &	24.0    &	3     	\\
J1747$-$2958	 & r  $^o$     &	359.3   & $-$0.8    &	 98.8    &	61.3	&	  26 &		251 &	23.5   &  0.25	\\
J1809$-$2332	 & g  $^b$  & 7.4   &	 $-$2.0  &	 147    &	  34.4 &	68		    &		  43.0    &	  	6.5	  &	 $^{2,3}\,<0.06$    	\\
J1813$-$1246	 & g  $^b$     & 17.2    &  2.4     &	  48.1    &	  17.6		       &	  43		    &		626 &	76.2    &	$^2\,<0.2$ \ 	   	\\
J1826$-$1256	 & g  $^b$     &	18.5    &	 $-$0.4    &110    &	121		&	  14		    &		358&	25.2    &	$^{2,3}\,<0.06$ 	\\
J1833$-$1034	 & r  $^o$     &	21.5    &	 $-$0.9  &	 61.9    &	      	202	&	    5	&	       3370&	137.3   &		  0.07   		\\
J1836$+$5925	 & g  $^b$     &	 88.9    &	       25.0    &	   173   &	    1.5	  &  1800	  &		    1.2     &	  	0.9	  &	     $^4\,<0.007$  		\\
J1907$+$06	   & g  $^{b,r}$   &40.2    & $-$0.9    &	   107   &	  87.3	   &	  19		    &		284 &	23.2    &		 $<0.02$ 		\\
J1952$+$3252	 & r  $^n$     & 68.8    &  2.8     &	 39.5    &	5.8	 &	110 	 &		374 &	71.6    &		  1   	\\
J1958$+$2846	 & g  $^b$     & 65.9    & $-$0.2    &	290   &	222		&	  21  &		35.8    &	  	3.0	  &		  ...   		\\
J2021$+$3651	 & r  $^p$     &	75.2    &	  0.1     &	   104   &	  95.6  &	  17	  &		338 &	26.0    &		  0.1 \      	\\
J2021$+$4026	 & g  $^{b,s}$   &	 78.2    &	 2.1     &	   265    &	  54.8   &	  77		    &		  11.6    &	  	1.9	  &	 	  ... 		\\
J2032$+$4127	 & g  $^{b,t}$   &	 80.2    &1.0     &	   143     &	  19.6	 &	120		&		26.3    &	  	5.3	  &	   $^2\,$ 0.24   		\\
J2043$+$2740	 & r  $^q$  & 70.6  &  $-$9.2    &	96.1    &	  1.3   &       1200		    &		    5.6  &	3.6	  &	 7	\\
J2124$-$3358	 & m  $^d$  &	  10.9    &	 $-$45.4   &	4.9    &  12$\times 10^{-6}$  &	0.6$\times 10^{6}$ & 0.4    &		18.8    &		  1.6 \      	\\
J2229$+$6114	 & r  $^m$     & 106.6   &	 2.9  &51.6  	&	  78.3	 &	    11	&	  2250 &	134.5   &		  0.25 	\\
J2238$+$59	   & g  $^b$     &	  106.5   & 0.5   &	163 &	  98.6	&	    26		    &		  90.3    &	  	8.6	  & ...		\\
\hline
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/DistanceTable.tex <==
% \table{tab:dist}
%
% Teresa M. \& Peter D. - 28 July 2009 
% PeterH - 31 July 2009
% ECF - 1 Aug 2009
%
% DAS - 2 Aug 2009: break Table out into a separate file
% 
% 
% Incorporated comments from F. Camilo - 22 Aug 2009
% Comments from FC not yet addressed are:
% 
% Maybe make title of table more specific.
% _______________
% Give numbers with sensible precision: e.g., 2.07_{-1.07}^{+1.38} should
% become 2.1_{-1.1}^{+1.4} - at least in the table, even if you want to
% use higher precision for figures.  All these digits just make the table
% busier, and in reality this is fake precision.
% _______________
% As I mentioned before, I think the values for J1747 and J2032 should
% be changed (and the 'Method' would be a combination of DM and other).
% And those are just two near and dear to my heart, I wonder if others
% could likewise be improved...
% _______________
% I don't understand why you use individual references for all the DMs -
% why not just the ATNF catalog ref?  I mean, you do that for S_1400 in
% Table 2.  (where possible, naturally). 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%inizio variazioni
\begin{scriptsize}
\begin{tabular}{lcc}
\hline
\hline
Nom du Pulsar & Distance (kpc) & Méthode \\
\hline
J0007+7303     &    1.4$\pm$0.3 	    & HI    \\% Pineault, S., et al., 1993, AJ, 105, 1060 \\	     
J0030+0451     &    0.300$\pm$0.090	    & P    \\% Lommen, A.N., et al., 2006, ApJ, 642, 1012 \\	      
J0205+6449     &    2.6--3.2		    & HI       \\% Green & Gull 1982; Roberts,D.A., et al., 1993, A\&A, 274, 438 (a) \\    
J0218+4232     &    2.5--4		    & A      \\ %Bassa et al 2003	   
J0248+6021     &    2--9		    & A    \\ %Cognard private communication	     \\ 	 
J0437$-$4715   &    0.1563$\pm$0.0013	    & P    \\% Deller et al. 2008 \\	   
J0534+2200     &    2.0$\pm$0.5 	    & A     \\% Trimble 1973 \\  	       
J0613$-$0200   &    0.48$^{+0.19}_{-0.11}$    & P       \\% Hotan, A. W, et al., 2006, MNRAS, 369, 1502  \\      
J0631+1036     &    0.75--3.62  	     & A    \\%Zepka, A., et al., 1996, ApJ, 456, 305 (b)  \\	     
J0633+1746     &    0.250$^{+0.120}_{-0.062}$ & P    \\%Faherty et al. 2007 \\  	
J0659+1414     &    0.288$^{ +0.033}_{-0.027}$ & P     \\% Brisken, W. F., et al., 2003, ApJ, 593, 89 \\      
J0742$-$2822   &    2.07$^{+1.38}_{-1.07}$    & DM    \\%Koribalski, B., et al.,1995, ApJ, 441, 756 (c)   \\   
J0751+1807     &    0.6$^{ +0.6}_{-0.2}$      & P    \\%Nice et al. 2005\\
J0835$-$4510   &    0.287$^{+0.019}_{-0.017}$ & P     \\%Dodson, R. et al., 2003, ApJ, 596, 1137 \\	     
J1028$-$5819   &    2.33$\pm$0.70	    & DM    \\%Keith, M.J., et al. 2008, MNRAS, 389, 1881 (d) \\     
J1048$-$5832   &    2.71$\pm$0.81	    & DM    \\%Johnston s., et al., 1996, MNRAS, 279, 661 (b) \\     
J1057$-$5226   &    0.72 $\pm$0.2	    & DM   \\%Weltevrede \& Wright 2009 \\    
J1124$-$5916   &    4.8$^{+0.7}_{-1.2 }$      & A    \\%Gonzalez, M., Safi-Harb, S., 2003, ApJ, 583, 91 \\  
J1418$-$6058   &    2--5		    & A     \\%Ng et al 2005;  Yadigaroglu & Romani 1997	  
J1420$-$6048   &    5.6$\pm$1.7 	    & DM  \\%D'amico et al 2001 ApJ...552L..45D
J1509$-$5850   &    2.6$\pm$0.8 	    & DM  \\% Hui, C.Y., Becker, W., 2007, A\&A,470, 965 (b); 25% error \\	 
J1614$-$2230   &    1.27$\pm$0.39	    & DM   \\%Crawford, F., et al., 2006, ApJ, 652, 1499 (d) \\     
J1709$-$4429   &    1.4--3.6		    & A     \\%McGowan et al 2004;Koribalski B., et al., 1995, ApJ, 441, 756 (c) \\	  
J1718$-$3825   &    3.82$\pm$1.15	   & DM   \\%Manchester, R.N., et al., 2001, MNRAS, 328, 17 (b) \\ 
J1741$-$2054   &    0.38$\pm$0.11	    & DM   \\%Camilo et al 2009 \\	
J1744$-$1134   &    0.357$^{+0.043}_{-0.035}$ & P     \\%Toscano, M., et al., 1999, ApJ, 523, 171 \\	     
J1747$-$2958   &    2.0$\pm$0.6 	    & DM   \\%Camilo, F., et al., 2002a, ApJ, 579, 25 (d) \\	      
J1809$-$2332   &    1.7$\pm$1.0 	    & HI   \\%Oka et al 1999
J1833$-$1034   &    4.7$\pm$0.4 	    & HI    \\%Camilo, F., et al., 2006, ApJ, 637, 456 \\	     
J1836+5925     &    $<$0.8		    & A      \\%Halpern, Camilo and Gotthelf 2007 ApJ 668 1154		     
J1952+3252     &    2.0$\pm$0.5 	    & HI   \\%Greidanus, H., Strom, R.G., 1990, A\&A, 240, 376 \\    
J2021+3651     &    2.1$^{+2.1}_{-1.0}$       & A    \\%Van Etten, A., et al., 2008, ApJ, 680, 1417 \\ 	 
J2021+4026     &    1.5$\pm$0.45	    & HI    \\%Landecker et al 1980, AASS 39 133 	     
J2032+4127     &    3.6$\pm$1.08	    & DM      \\%Camilo 2009 \\		       
J2043+2740     &    1.80$\pm$0.54	    & DM      \\%Ray, W., et al., 1996 apj 470 1103 \\	     
J2124$-$3358   &    0.25$^{+0.25}_{-0.08}$    & P    \\%Hotan et al 2006    \\  
J2229+6114     &    0.8--6.5		    & A    \\%Kothes et al 2001; Halpern, J.P.,  et al., 2001b, ApJ, 547, 323 (e) \\   
\hline
\hline
%\tablenotetext{a}{K distance evaluation from kinematic model; P from parallax; DM from dispersion measure using the \citet{Cordes2002} model; O from other measurements. For DM measurements, we assume a minimum distance uncertainty of 30\%, as discussed in Section 3.1}
%\tablenotetext{b}{For DM, the reference gives the DM measurement.}
%\tablecomments{The best known distances of 37 pulsars detected by Fermi. 9 of the pulsars in the catalog have no distance estimate and are not included in this table.}


%\tablerefs{
%(1)  \citet{Bassa2003};
%(2)  \citet{Brisken2003};
%(3)  \citet{Camilo2009};
%(4)  \citet{Camilo2006}; 
%(5)  \citet{Camilo2002a};          
%(5)  \citet{Gaensler2004};          
%(6)  \citet{Cognard2009};
%(7)  \citet{Crawford2006};
%(8)  \citet{DAmico2001};
%(9)  \citet{Deller2008};
%(10)  \citet{Dodson2003};
%(11) \citet{Faherty2007};
%(12) \citet{Gonzalez2003};
%(13) \citet{Green1982};
%(14) \citet{Greidanus1990};
%(15) \citet{Halpern2007};   
%(16) \citet{Halpern2001a};                                                      
%(17) \citet{Hotan2006};
%(18) \citet{Hui2007};
%(19) \citet{Keith2008};
%(20) \citet{Koribalski1995};
%(21) \citet{Kothes2001};
%(22) \citet{Johnston1996};
%(23) \citet{Landecker1980};
%(24) \citet{Lommen2006}; 
%(25) \citet{Manchester2001};
%(26) \citet{McGowan2004};
%(27) \citet{Ng2005};  
%(28) \citet{Nice2005};
%(29) \citet{Oka1999};
%(30) \citet{Pineault1993};  
%(31) \citet{Ray1996};       
%(32) \citet{Roberts1993}; 
%(33) \citet{Toscano1999};
%(34) \citet{Trimble1973};
%(35) \citet{VanEtten2008};
%(36) \citet{Weltevrede2009};
%(37) \citet{Yadigaroglu1997};
%(38) \citet{Zepka1996}
%  }              
\end{tabular}
\end{scriptsize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%fine variazioni


==> tableaux/LAT_performance.tex <==
\begin{tabular}{ll}
\hline 
\hline
Paramètres & Valeur ou intervalle \\
\hline
Intervalle en énergie & 0.02\ --\ 300 GeV \\
Surface efficace à incidence normale & \\
\ \ 0.1\ --\ 10\,GeV & 7000\,cm$^{2}$ \\
\ \ 10\ --\ 300\,GeV & 8000\,cm$^{2}$ \\
Résolution en énergie (1$\sigma$ gaussien): & \\
\ \ 0.1\ --\ 10\,GeV sur l'axe & $\leq$ 10\% \\
\ \ 10\ --\ 300\,GeV sur l'axe & $\leq$ 20\% \\
\ \ $>$ 10\,GeV (à $>$60\,$^{\circ}$ d'incidence) & $\leq$ 6\% \\
Résolution angulaire (rayon de confinement de 68\%): & \\
\ \ $>$ 10\,GeV & $\leq$ 0.15\degr \\
\ \ 1\,GeV      & 0.5\degr \\
\ \ 100\,MeV    & 3.5\degr \\
Champ de vue & 2.4 sr \\
Précision temporelle & $<$ 1 $\mu$sec \\
Temps mort & 26.5 $\mu$sec \\
\hline
\hline
\end{tabular}

==> tableaux/associations.tex <==
% \table{tbl-assoc}
%
% Incorporated comments from F. Camilo - 22 Aug 2009
% Comments from FC not yet addressed are:
% 
% In positional associations, J2032+4127 should also have HEGRA TeV J2032+4130
% - or just TeV J2032+4130 against it.  I'm going to guess that this column
% is incomplete. 
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%inizio variazioni

\begin{tiny}
\begin{tabular}{lclll}
\hline
\hline
PSR & Nom Alternatif & Association$^a$ BSL & Associations EGRET$^b$ & Associations Objets \\
\hline
J0007$+$7303 	& ... 			& 0FGL J0007.4$+$7303 & 3EG J0010+7309 		& CTA 1 \\
   				&   				&   					& EGR J0008$+$7308 	& PWN G119.5$+$10.2 $^{1}$ \\
J0030$+$0451 	& ... 			& 0FGL J0030.3$+$0450 & EGR J0028$+$0457 	& ... \\
J0205$+$6449 	& ... 			& ... 				& ... 				& 3C 58 $^{2}$ \\
   				&   				&   					&   					& PWN G119.5$+$10.2 $^{1}$ \\
J0218$+$4232 	& ... 			& ... 				& ... 				& ... \\
J0248$+$6021 	& ... 			& ... 				& ... 				& ... \\
J0357$+$32 		& ... 			& 0FGL J0357.5$+$3205 & ... 				& ... \\
J0437$-$4715 		& ... 			& ... 				& ... 				& PWN G253.4$-$42.0 $^{1}$ \\
J0534$+$2200 	& Crab 			& 0FGL J0534.6$+$2201 & 3EG J0534$+$2200 	& PWN/SNR G184.6$-$5.8 $^{1}$ \\
   				& PSR B0531$+$21 &   					& EGR J0534$+$2159 	& HESS J0534$+$220 $^{4}$ \\
J0613$-$0200 		& ... 			& 0FGL J0613.9$-$0202 	& ... 				& ... \\
J0631$+$1036 	& ... 			& 0FGL J0631.8$+$1034 & ... 				& ... \\
J0633$+$0632 	& ... 			& 0FGL J0633.5$+$0634 & 3EG J0631$+$0642 	& ... \\
   				&   				&   					& EGR J0633$+$0646 	&   \\
J0633$+$1746 	& Geminga 		& 0FGL J0634.0$+$1745 & 3EG J0633$+$1751 	& PWN G195.1$+$4.3 $^{1}$ \\
   				&   				&   					& EGR J0633$+$1750 	& MGRO J0632$+$17 $^{3,11}$ \\
J0659$+$1414 	& PSR B0656$+$14 & ... 				& ... 				& SNR 203.0$+$12.0 \\
J0742$-$2822 		& PSR B0740$-$28 	& ... 				& ... 				& ... \\
J0751$+$1807 	& ... 			& ... 				& ... 				& ... \\
J0835$-$4510 		& Vela 			& 0FGL J0835.4$-$4510 	& 3EG J0834$-$4511 	& PWN G263.9$-$3.3 $^{1}$ \\
   				& PSR B0833$-$45 &   					& EGR J0834$-$4512	& HESS J0835$-$455 $^{5}$ \\
J1028$-$5819 		& ... 			& 0FGL J1028.6$-$5817 	& 3EG J1027$-$5817 	& ... \\
J1048$-$5832 		& PSR B1046$-$58 & 0FGL J1047.6$-$5834 	& 3EG J1048$-$5840 	& PWN G287.4$+$0.58 $^{1}$ \\
   				&   				&   					& EGR J1048$-$5839	&   \\
J1057$-$5226 		& PSR B1055$-$52 & 0FGL J1058.1$-$5225 	& 3EG J1058$-$5234 	& ... \\
   				&   				&   					& EGR J1058$-$5221 	&   \\
J1124$-$5916 		& ... 			& ... 				& ... 				& MSH 11$-$54 \\
   				&   				&   					&   					& PWN/SNR G292.0$+$1.8 $^{1,2}$ \\
J1418$-$6058 		& ... 			& 0FGL J1418.8$-$6058 	& 3EG J1420$-$6038 	& PWN G313.3$+$0.1 $^{1}$ \\
   				&   				&   					&   					& HESS J1418$-$609 $^{6}$ \\
J1420$-$6048 		& ... 			& ... 				& 3EG J1420$-$6038 	& PWN G313.6$+$0.3 $^{1}$ \\
   				&   				&   					& EGR J1418$-$6040 	& HESS J1420$-$607 $^{6}$ \\
J1459$-$60 		& ... 			& 0FGL J1459.4$-$6056 	& ... 				& ... \\
J1509$-$5850$^c$ 		& ... 			& 0FGL J1509.5$-$5848 	& ... 				& PWN G319.97$-$0.62 $^{1}$ \\
J1614$-$2230 		& ... 			& ... 				& 3EG J1616$-$2221 	& ... \\
J1709$-$4429 		& PSR B1706$-$44 & 0FGL J1709.7$-$4428 	& 3EG J1710$-$4439 	& PWN G343.1$-$2.3 $^{1}$ \\
   				&   				&   					& EGR J1710$-$4435	& HESS J1708$-$443 $^{7}$ \\
J1718$-$3825 		& ... 			& ... 				& ... 				& HESS J1718$-$385 $^{8}$ \\
J1732$-$31 		& ... 			& 0FGL J1732.8$-$3135 	& 3EG J1734$-$3232 	& ... \\
   				&   				&   					& EGR J1732$-$3126	&   \\
J1741$-$2054 		& ... 			& 0FGL J1742.1$-$2054 	& 3EG J1741$-$2050 	& ... \\
J1744$-$1134 		& ...  		& ... 				& ... 				& ... \\
J1747$-$2958 		& ... 			& ... 				& ... 				& PWN G359.23$-$0.82 $^{1}$ \\
J1809$-$2332 		& ... 			& 0FGL J1809.5$-$2331 	& 3EG J1809$-$2328 	& PWN G7.4$-$2.0 $^{1}$ \\
J1813$-$1246 		& ... 			& 0FGL J1813.5$-$1248 	& GeV J1814$-$1228 	& ... \\
J1826$-$1256 		& ... 			& 0FGL J1825.9$-$1256 	& 3EG J1826$-$1302 	& PWN G18.5$-$0.4 $^{1}$ \\
J1833$-$1034 		& ... 			& ... 				& ... 				& PWN G21.5$-$0.9 $^{1}$ \\
   				&   				&   					&   					& HESS J1833$-$105 $^{9}$ \\
J1836$+$5925 	& ... 			& 0FGL J1836.2$+$5924 	& 3EG J1835$+$5918 	& ... \\
J1907$+$06 		& ... 			& 0FGL J1907.5$+$0602 	& GeV 1907$+$0557 	& MGRO J1908$+$063 $^{3}$ \\
   				&   				&   					&   					& HESS J1908$+$06 $^{10}$ \\
J1952$+$3252 	& PSR B1951$+$32 & 0FGL J1953.2$+$3249 & ... 				& CTB 80 \\
   				&   				&   					&   					& PWN G69.0$+$2.7 $^{1}$ \\
J1958$+$2846 	& ... 			& 0FGL J1958.1$+$2848 & 3EG J1958$+$2909 	& ... \\
J2021$+$3651 	& ... 			& 0FGL J2020.8$+$3649 & ... 				& PWN G75.2$+$0.1 $^{1}$ \\
   				&   				&   					&   					& MGRO J2019$+$37 $^{3}$ \\
J2021$+$4026 	& ... 			& 0FGL J2021.5$+$4026 & 3EG J2020$+$4017 	& $\gamma$ Cygni \\
   				&   				&   					&   					& SNR G078.1$+$01.8 $^{2}$ \\
J2032$+$4127 	& ... 			& 0FGL J2032.2$+$4122 & 3EG J2033$+$4118 	& MGRO J2031$+$41 $^{3}$ \\
   				&   				&   					& EGR J2033$+$4117 	&   \\
J2043$+$2740 	& ... 			& ... 				& ... 				& ... \\
J2124$-$3358 		& ... 			& 0FGL J2124.7$-$3358 	& ... 				& PWN G10.9$-$45.4 $^{1}$ \\
J2229$+$6114 	& ... 			& 0FGL J2229.0$+$6114 & 3EG J2227$+$6122 	& PWN G106.6$+$2.9 $^{1}$ \\
   				&   				&   					& EGR J2227$+$6114 	& MGRO J2228$+$61  $^{3,11}$ \\
J2238$+$59 		& ... 			& ... 				& ... 				& ... \\
\hline
\hline
%\tablenotetext{a}{Source designator from the LAT Bright Source List \citep{BSL}.}
%\tablenotetext{b}{Source designator(s) from the 3rd EGRET \citep[3EG: ][]{3rdCat}, Revised EGRET \citep[EGR: ][]{EGRcatalog}  and/or GeV Point Source \citep[GeV: ][]{Lamb1997} catalogs.} 
%\tablenotetext{c}{Note that this is not PSR B1509-58 seen with \textit{CGRO}.}


%\tablecomments{Alternate names for the pulsars in this catalog are given in column 2, while the LAT Bright Source List designation is provided in column 3. Column 4 shows positional associations with cataloged EGRET sources. Finally, positional associations with SNRs, PWNe and selected TeV sources are provided.}

%\tablerefs{{1. \citet{Roberts2005}}, {2. \citet{Green2009}}, {3. \citet{Milagro2009}}, {4. \citet{HESSCrab2006}}, {5. \citet{HESSVela2006}}, {6.
%\citet{HESSRabbit2006}}, {7. \citet{HESS1709_2009}}, {8. \citet{HESS1718_2007}}, {9. \citet{HESS1833_2007}}, {10. \citet{HESS1908_2009}}, {11.\citet{ATEL2172} }}

\end{tabular}
\end{tiny}

==> tableaux/cal_performance.tex <==
\begin{tabular}{ll}
\hline 
\hline
Caractéristiques & Performance \\
\hline
Profondeur, incluant le trajectographe & 10.1 X$_{0}$ \\
Stabilité des voies actives & $>$ 99\% en 5 ans \\
Gamme d'énergie & 20\,MeV - $>$\,300\,GeV \\
Résolution en énergie & $<$ 20\% à 2\,MeV $<$ E $<$ 100\,MeV \\
...										& $<$ 10\% à 100\,MeV $<$ E $<$ 10\,GeV \\
... $\theta >$60\degr & $\leq$ 6\% à 10\,GeV $<$ E $<$ 100\,GeV \\
\hline
\hline
\end{tabular}

==> tableaux/cgropsr.tex <==
\begin{scriptsize}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{cccccccc}
\hline 
\hline
Nom & Période & $\tau$ & $\dot{E}$ & $F_{E}$ & $d$ & $L_{\gamma}$ & $\eta$ \\
    &   (s)   & (ky)   & (erg\,s$^{-1}$) & (erg\,cm$^{-2}$\,s$^{-1}$) & (kpc) & (erg\,s$^{-1}$) & (E$>$1\,eV) \\
\hline
Crab, J0534+2200 & 0.033 & 1.3 & $4.5 \times 10^{38}$ & $1.3 \times 10^{-8}$ & 2.0 & $5.0 \times 10^{35}$ & 0.001 \\ 
B1509$-$58 & 0.150 & 1.5 & $1.8 \times 10^{37}$ & $8.8 \times 10^{-10}$ & 4.4 & $1.6 \times 10^{35}$ & 0.009 \\ 
Vela, J0835$-$4510 & 0.089 & 11 & $7.0 \times 10^{36}$ & $9.9 \times 10^{-9}$ & 0.3 & $8.6 \times 10^{33}$ & 0.001 \\ 
J1709$-$4429, B1706$-$44 & 0.102 & 17 & $3.4 \times 10^{36}$ & $1.3 \times 10^{-9}$ & 2.3 & $6.6 \times 10^{34}$ & 0.019 \\
J1952+3252, B1951+32 & 0.040 & 110 & $3.7 \times 10^{36}$ & $4.3 \times 10^{-10}$ & 2.5 & $2.5 \times 10^{34}$ & 0.007 \\
Geminga, J0633+1746 & 0.237 & 340 & $3.3 \times 10^{34}$ & $3.9 \times 10^{-9}$ & 0.16 & $9.6 \times 10^{32}$ & 0.029 \\
J1057$-$5226, B1055$-$52 & 0.197 & 530 & $3.0 \times 10^{34}$ & $2.9 \times 10^{-10}$ & 0.72 & $1.4 \times 10^{33}$ & 0.048 \\
\hline
J1048$-$5832, B1046$-$58 & 0.124 & 20 & $2.0 \times 10^{36}$ & $3.7 \times 10^{-10}$ & 2.7 & $2.6 \times 10^{34}$ & 0.013 \\
J0659+1414, B0656$+$14 & 0.385 & 100 & $4.0 \times 10^{34}$ & $1.6 \times 10^{-10}$ & 0.3 & $1.3 \times 10^{32}$ & 0.003 \\
J0218+4232 & 0.002 & 460000 & $2.5 \times 10^{35}$ & $9.1 \times 10^{-11}$ & 2.7 & $6.4 \times 10^{33}$ & 0.026 \\
\hline
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/ephemeris_j0205.tex <==
\begin{tabular}{ll}
\hline 
\hline
Paramètres & Valeurs \\
\hline
Ascension Droite (J2000)\dotfill & 02$^{h}$05$^{m}$37.92$^{s}$ \\
Déclinaison (J2000)\dotfill & +64${^\circ}$49'42.8000014'' \\
Fréquence F0 (s$^{-1}$)\dotfill & 15.2144837749(6) \\
F1 (s$^{-2}$)\dotfill & -4.48200(5) $\times$10$^{-11}$ \\
F2 (s$^{-3}$)\dotfill & -1.43(2) $\times$10$^{-20}$ \\
F3 (s$^{-4}$)\dotfill & -2.7(5) $\times$10$^{-28}$ \\
F4 (s$^{-5}$)\dotfill & 6.22(7) $\times$10$^{-33}$ \\
F5 (s$^{-6}$)\dotfill & 2.05(6) $\times$10$^{-33}$ \\
F6 (s$^{-7}$)\dotfill & -1.43(1) $\times$10$^{-47}$ \\
F7 (s$^{-8}$)\dotfill & -7.3(1) $\times$10$^{-52}$ \\
Epoque, T$_0$ (MJD[TDB])\dotfill & 54767.0 \\
Date de référence pour le $\phi_{0}$ (MJD[TDB])$^{a}$\dotfill & 54768.07703065005798 \\
Intervalle de validité en MJD \dotfill & 54634.253 -- 54899.693 \\
Nombre de TOAs\dotfill & 68 \\
Mesure de dispersion, DM(cm$^{-3}$\,pc)\dotfill & 140.7 $\pm$ 0.3 \\
Modèle d'éphéméride du S.S. \dotfill & DE405\\
\hline
\hline
\end{tabular}

==> tableaux/ephemeris_j1048.tex <==
\begin{tabular}{ll}
\hline 
\hline
Paramètres & Valeurs \\
\hline
Ascension Droite (J2000)\dotfill & 22$^{h}$29$^{m}$05.28000084$^{s}$ \\
Déclinaison (J2000)\dotfill & +61${^\circ}$14'09.3000042'' \\
Fréquence (s$^{-1}$)\dotfill & 8.08403505(1) \\
Dérivée première de la fréquence (s$^{-2}$)\dotfill & -6.282(1) $\times$10$^{-12}$ \\
Epoque, T$_0$ (MJD[TDB])\dotfill & 54575.0 \\
Date de référence pour le $\phi_{0}$ (MJD[TDB])$^{a}$\dotfill & 54743.974102133058178 \\
Intervalle de validité en MJD \dotfill & 54565.3 -- 54931.3 \\
Nombre de TOAs\dotfill & 20 \\
Mesure de dispersion, DM(cm$^{-3}$\,pc)\dotfill & 128.822 $\pm$ 0.008 \\
Modèle d'éphéméride du S.S. \dotfill & DE405\\
\hline
\hline
\end{tabular}

==> tableaux/highlevelcut.tex <==
\begin{scriptsize}
\begin{tabular}{ll}
\hline 
\hline
Nom de la coupure & Définition \\
\hline
Coupures minimes & TkrNumTracks$>$0 \&\& CalCsIRLn$>$4 \&\& CalEnergyRaw$>$5 \vspace{0.2cm} \\
Transient & CTBCORE$>$0. \&\& CTBBestEnergyProb$>$0. \&\& CTBBestEnergy$>$10 \\
				  & \&\& CTBBestEnergyRatio$<$5 \&\& \textbf{CTBClassLevel$>$0} \vspace{0.2cm} \\

Source    & CTBCORE$>$0.1 \&\& CTBBestEnergyProb$>$0.1 \&\& CTBBestEnergy$>$10 \\
          & \&\&  CTBBestEnergyRatio$<$5 \&\& \textbf{CTBClassLevel$>$1} \vspace{0.2cm} \\

Diffuse   & CTBCORE$>$0.1 \&\& CTBBestEnergyProb$>$0.1 \&\& CTBBestEnergy$>$10 \\
					& \&\& CTBBestEnergyRatio$<$5 \&\& \textbf{CTBClassLevel$>$2} \\
ROI       & (FT1Dec$-$dec)$^{2}$+(cos(FT1Dec*$\pi$/180)*(FT1Ra$-$ra))$^{2}$<100 \\
\hline
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/luminosity.tex <==
\begin{tabular}{lccccc}
\hline 
\hline
Pulsar & Luminosité X$^{a}$ & Luminosité $\gamma$ & L$_{X}$/L$_{\gamma}$ & $\tau$ & Réfs. \\
       & L$_{X}$ (erg\,s$^{-1}$) & L$_{\gamma}$ (erg\,s$^{-1}$) &  & (an) & \\
\hline
Crab\dotfill & 1.55 $\times$ 10$^{36}$ & 6.2 $\times$ 10$^{35}$ & 2.5 & 1300 & 1,2 \\
B1509$-$58$^{b}$\dotfill & 1.09 $\times$ 10$^{35}$ & 1.6 $\times$ 10$^{35}$ & 0.7 & 1500 & 1,2 \\
J0205$+$6449\dotfill & 1.51 $\times$ 10$^{33}$ & 6.1 $\times$ 10$^{34}$ & 2.5 $\times$ 10$^{-2}$ & 5400 & 1,6 \\
J2229$+$6114\dotfill & 6.76 $\times$ 10$^{32}$ & 2.6 $\times$ 10$^{35}$ & 2.6 $\times$ 10$^{-3}$ & 10500 & 1,7 \\
Vela\dotfill & 3.02 $\times$ 10$^{31}$ & 8.7 $\times$ 10$^{34}$ & 3.5 $\times$ 10$^{-4}$ & 11000 & 1,4 \\
J2021+3651$^{c}$\dotfill & 9.19 $\times$ 10$^{32}$ & 8.2 $\times$ 10$^{35}$ & 1.1 $\times$ 10$^{-4}$ & 17000 & 3,5 \\
B1706-44\dotfill & 1.10 $\times$ 10$^{32}$ & 2.9 $\times$ 10$^{35}$ & 3.8 $\times$ 10$^{-4}$ & 17000 & 1,2 \\
J1048-5832\dotfill & 2.6 $\times$ 10$^{31}$	& 2.1	$\times$ 10$^{35}$ & 1.2 $\times$ 10$^{-4}$ & 20400 &	1,7 \\
\hline
\hline
\end{tabular}

==> tableaux/psr1048and2229.tex <==
\begin{footnotesize}
\begin{tabular}{llcc}
\hline 
\hline
Analyse & Paramètres & PSR~J1048$-$5832 & PSR~J2229+6449  \\
\hline
\vspace{0.2mm}
\textbf{Temporelle}   & Nombre de photons pulsés & 933 $\pm$ 93 & 1365 $\pm$ 97\\
       & Position des pics ($\phi$)& 0.15 $\pm$ 0.01 $\pm$ 0.0001 (P1) & 0.49 $\pm$ 0.01 $\pm$ 0.001 \\
       &              & 0.57 $\pm$ 0.01 $\pm$ 0.0001 (P2) & \\
       & Séparation des pics ($\Delta$) & 0.42 $\pm$ 0.01 $\pm$ 0.0001 & \\
       & FWHM(pic)    & 0.06 $\pm$ 0.01 (P1) & 0.23 $\pm$ 0.03 \\
       &              & 0.10 $\pm$ 0.02 (P2) &  \\
\hline
\vspace{0.2mm}
       \textbf{Spectrale}
       & $^{a}$F (10$^{-7}$ cm$^{-2}$s$^{-1}$) & 2.19 $\pm$ 0.22 $\pm$ 0.32 & 3.77 $\pm$ 0.22 $\pm$ 0.44 \\
       & $^{b}$F$_{E}$ (10$^{-11}$ erg cm$^{-2}$s$^{-1}$) & 19.4 $\pm$ 1.0 $\pm$ 3.1 & 23.7 $\pm$ 0.7 $\pm$ 2.5 \\
       & $\Gamma$& 1.38 $\pm$ 0.06 $\pm$ 0.12 & 1.85 $\pm$ 0.06 $\pm$ 0.10 \\
       & $^{c}$E$_{c}$ (GeV)& 2.3$^{+0.3}_{-0.4}$ $\pm$ 0.3 & 3.6$^{+0.9}_{-0.6}$ $\pm$ 0.6 \\
       & L$_{\gamma}$ (10$^{35}$ erg s$^{-1}$) & 2.1 $f_{\Omega}$ (d/3kpc)$^{2}$ & 2.6 $f_{\Omega}$ (d/3kpc)$^{2}$ \\
       & $\eta_{\gamma}$ & 0.10 $f_{\Omega}$ (d/3kpc)$^{2}$& 0.011 $f_{\Omega}$ (d/3kpc)$^{2}$ \\\hline
\hline
\end{tabular}
\end{footnotesize}

==> tableaux/pulsepar.tex <==
% \table{tbl-pulse}
%
% Incorporated comments from F. Camilo - 22 Aug 2009
% Comments from FC not yet addressed are:
% 
% Peak multiplicity:  how was this obtained?  I don't believe it's
% ever mentioned in text; by eye? by a fit of Gaussians, Lorentzians, what
% have you?  how did you decide 2 were enough, and 3 were not needed?  were
% you looking at the chi sq. of the fit, at residuals?  Somewhere in text
% this should be explained.
% _______________
% Radio lag uncertainties: have they all taken into account DM uncertainty?
% I'm not sure that for J1741-2054 has.  If there's a 'b' footnote for a
% couple of pulsars where it's not clear whether 1 or 2 peaks describe the
% profile, how about a reference for J1741, where Camilo et al. (2009b) claim
% 3 peaks?  At least mention that it's not clear whether it has 2 or 3, and
% give that ref - lest the unsuspecting reader come to believe on the basis
% of this table that all pulsars has 1 or 2 peaks.
% _______________
% As I already mentioned, why only one off-pulse range for all pulsars,
% when this doesn't describe many of them?
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  
\begin{scriptsize}
\begin{tabular}{llcccc}
%\tablewidth{0pt}
%\tablecaption{Pulse shape parameters of LAT-detected pulsars
%\label{tbl-pulse}}
\hline
\hline
PSR & Type$^a$ & Multiplicité & Décalage Radio & Séparation des Pics $\gamma$ & Définition OFF  \\
    &          & des pics     & $\delta$       & $\Delta$                     & $\phi$ \\
\hline    
 J0007$+$7303	  &	    g  &  2  &  ...		 &  0.23 $\pm$ 0.01 & 0.29 -- 0.87 \\
 J0030$+$0451	  &	    m  &  2  &  0.18 $\pm$ 0.01  &  0.44 $\pm$ 0.01 & 0.68 -- 0.12 \\
 J0205$+$6449	  &	    r  &  2  &  0.08 $\pm$ 0.01  &  0.50 $\pm$ 0.01 & 0.64 -- 0.02 \\
 J0218$+$4232	  &	    m &  2  &  0.32 $\pm$ 0.02  &  0.36 $\pm$ 0.02 & 0.84 -- 0.16 \\
 J0248$+$6021	  &	    r  &  1  &  0.35 $\pm$ 0.01  &  ... 	    & 0.71 -- 0.19 \\
 J0357$+$32	  	&	    g  &  1  &  ...		 &  ... 	    & 0.34 -- 0.86 \\
 J0437$-$4715	  	&	    m &  1  &  0.43 $\pm$ 0.02  &  ... 	    & 0.60 -- 0.20 \\
 J0534$+$2200	  &	    r  &  2  &  0.09 $\pm$ 0.01  &  0.40 $\pm$ 0.01 & 0.62 -- 0.98 \\
 J0613$-$0200	  	&	    m &  1  &  0.42 $\pm$ 0.01  &  ... 	    & 0.56 -- 0.16 \\
 J0631$+$1036	  &	    r  &  1  &  0.54 $\pm$ 0.02  &  ... 	    & 0.80 -- 0.20 \\
 J0633$+$0632	 &	    g  &  2  &  ...		 &  0.48 $\pm$ 0.01 & 0.09 -- 0.45 \\
 J0633$+$1746	  &	    g  &  2  &  ...		 &  0.50 $\pm$ 0.01 & 0.24 -- 0.54 \\
 J0659$+$1414	  &	    r  &  1  &  0.21 $\pm$ 0.01  &  ... 	    & 0.40 -- 1.00 \\
 J0742$-$2822	  	&	    r  &  1  &  0.61 $\pm$ 0.02  &  ... 	    & 0.84 -- 0.44 \\
 J0751$+$1807	  &	    m &  1  &  0.43 $\pm$ 0.02  &  ... 	    & 0.63 -- 0.99 \\
 J0835$-$4510	  	&	    r  &  2  &  0.13 $\pm$ 0.01  &  0.43 $\pm$ 0.01 & 0.66 -- 0.06 \\
 J1028$-$5819	  	&	    r  &  2  &  0.19 $\pm$ 0.01  &  0.47 $\pm$ 0.01 & 0.76 -- 0.12 \\
 J1048$-$5832	  	&	    r  &  2  &  0.15 $\pm$ 0.01  &  0.42 $\pm$ 0.02 & 0.64 -- 0.04 \\
 J1057$-$5226	  	&	    r  &  2  &  0.35 $\pm$ 0.05  &  0.20 $\pm$ 0.07 & 0.72 -- 0.20 \\
 J1124$-$5916	  	&	    r  &  2  &  0.23 $\pm$ 0.01 &  0.49 $\pm$ 0.01 & 0.60 -- 0.96 \\
 J1418$-$6058	  	&	    g  &  2  &  ...		 &  0.47 $\pm$ 0.01 & 0.54 -- 0.90 \\
 J1420$-$6048	  	&	    r  &  2$^b$ &  0.26 $\pm$ 0.02  &  0.18 $\pm$ 0.02 & 0.60 -- 0.10 \\
 J1459$-$60	  	&	    g  &  2  &  ...		 &  0.15 $\pm$ 0.03 & 0.34 -- 0.78 \\
 J1509$-$5850	  	&	    r  &  2$^b$ &  0.18 $\pm$ 0.03  &  0.20 $\pm$ 0.03 & 0.52 -- 1.00 \\
 J1614$-$2230	  	&	    m &  2  &  0.19 $\pm$ 0.01  &  0.51 $\pm$ 0.01 & 0.92 -- 0.14 \\
 J1709$-$4429	  	&	    r  &  2  &  0.24 $\pm$ 0.01  &  0.25 $\pm$ 0.01 & 0.66 -- 0.14 \\
 J1718$-$3825	  	&	    r  &  1  &  0.42 $\pm$ 0.02  &  ... 	    & 0.68 -- 0.20 \\
 J1732$-$31	  	&	    g  &  2  &  ...		 &  0.42 $\pm$ 0.02 & 0.49 -- 0.93 \\
 J1741$-$2054	  	&	    g  &  2  &  0.30 $\pm$ 0.01  &  0.18 $\pm$ 0.02 & 0.67 -- 0.19 \\
 J1744$-$1134	  	&	    m  &  1  &  0.83 $\pm$ 0.02  &  ... 	    & 0.08 -- 0.44 \\
 J1747$-$2958	  	&	    r  &  2  &  0.18 $\pm$ 0.01  &  0.42 $\pm$ 0.04 & 0.64 -- 0.10 \\
 J1809$-$2332	  	&	    g  &  2  &  ...		 &  0.35 $\pm$ 0.01 & 0.41 -- 0.89 \\
 J1813$-$1246	  	&	    g  &  2  &  ...		 &  0.47 $\pm$ 0.02 & 0.56 -- 0.90 \\
 J1826$-$1256	  	&	    g  &  2  &  ...		 &  0.47 $\pm$ 0.01 & 0.54 -- 0.94 \\
 J1833$-$1034	  	&	    r  &  2  &  0.15 $\pm$ 0.01  &  0.44 $\pm$ 0.01 & 0.68 -- 0.10 \\
 J1836$+$5925	  &	    g  &  2  &  ...		 &  0.48 $\pm$ 0.01 & ... \\
 J1907$+$06	  	&	    g  &  2  &  ...		 &  0.40 $\pm$ 0.01 & 0.46 -- 0.94 \\
 J1952$+$3252	  &	    r  &  2  &  0.15 $\pm$ 0.01  &  0.49 $\pm$ 0.01 & 0.68 -- 0.08 \\
 J1958$+$2846	  &	    g  &  2  &  ...		 &  0.45 $\pm$ 0.01 & 0.55 -- 0.95 \\
 J2021$+$3651	  &	    r  &  2  &  0.17 $\pm$ 0.01  &  0.47 $\pm$ 0.01 & 0.70 -- 0.04 \\
 J2021$+$4026	  &	    g  &  2  &  ...		 &  0.48 $\pm$ 0.01 & ... \\
 J2032$+$4127	  &	    g  &  2  &  0.15 $\pm$ 0.01  &  0.50 $\pm$ 0.01 & 0.60 -- 0.92 \\
 J2043$+$2740	  &	    r  &  2  &  0.20 $\pm$ 0.01  &  0.36 $\pm$ 0.01 & 0.64 -- 0.08 \\
 J2124$-$3358	  	&	    m  &  1  &  0.86 $\pm$ 0.02  &  ... 	    & 0.92 -- 0.58 \\
 J2229$+$6114	  &	    r  &  1  &  0.49 $\pm$ 0.01  &  ... 	    & 0.64 -- 0.14 \\
 J2238$+$59	  	&	    g  &  2  &  ...  &  0.50 $\pm$ 0.01 & 0.60 -- 0.92 \\
\hline
\hline
%\tablenotetext{a}{Types are r=radio-selected, g=gamma-selected, m=millisecond}
%\tablenotetext{b}{For some pulse profiles the current dataset does not allow clear discrimination between
%a single, broad pulse and two unresolved pulses. See the discussion in \citet{LAT6pulsars}
%regarding PSRs J1420$-$6048 and J1509$-$5850.}

%\tablecomments{~Light curve shape parameters evaluated from the full energy range light curve (see 
%Section 2.1.3). These include the peak multiplicity (3rd column), the lag $\delta$ of the first gamma 
%peak from the main radio peak for the radio-selected pulsars (4th column), and the phase difference 
%$\Delta$ between the main peaks (5th column). Column 6 lists the off-pulse phase range used in the 
%spectral analysis.}

\end{tabular}
\end{scriptsize}
%\normalsize


==> tableaux/tracker_performance.tex <==
\begin{tabular}{ll}
\hline 
\hline
Caractéristiques & Performance \\
\hline
Epaisseur d'une SSD & 0.4\,mm \\
Nombre de pistes par SSD & 384 \\
Distance séparant les pistes & 228\,${\mu}$m \\
Efficacité de déclenchement & >99\% \\
Pistes déclenchées par le bruit électronique & 10$^{-6}$ \\
Rapport hauteur/largeur & 0.4 \\
X$_{0}$ des 12 premiers plans convertisseurs (front) & 12 $\times$ 0.03 \\
X$_{0}$ des 4 derniers plans convertisseurs (back) & 4 $\times$ 0.18 \\
\hline
\hline
\end{tabular}
